Lower bounds for algebraic machines, semantically

This paper presents a new semantic method for proving lower bounds in computational complexity. We use it to prove that maxflow, a PTIME complete problem, is not computable in polylogarithmic time on parallel random access machines (PRAMs) working with integers, showing that NCZ \neq PTIME, where NCZ is the complexity class defined by such machines, and PTIME is the standard class of polynomial time computable problems (on, say, a Turing machine). On top of showing this new separation result, we show our method captures previous lower bounds results from the literature: Steele and Yao's lower bounds for algebraic decision trees, Ben-Or's lower bounds for algebraic computation trees, Cucker's proof that NC is not equal to PTIME on the reals, and Mulmuley's lower bounds for "PRAMs without bit operations".

==> IGmodels.tex <==
\section{Some models of computation}
\label{sec:some-models-comp}

We introduce different models of computation in the \amc framework, namely
Algebraic Computational Trees, Random Access Machines and Parallelized Random
Access Machines.

\subsection{Algebraic Computational Trees}
\label{sec:def-algebraic-computational-trees}

Algebraic computational trees follow the same principles as algebraic decision
trees, but they allow for the representation of computations as part of the tree.
I.e. one consider nodes for every algebraic operation on the set of polynomials.

More formally, an algebraic computational tree is defined from the nodes 
$\times$, $+$, $-$, $/$, $\sqrt{}$ and a test node with three sons corresponding 
to $<0$, $=0$ and $>0$ as in the algebraic decision trees case.

The difference is thus that algebraic computation trees only perform tests on
expression that are first defined by means of algebraic operations. If one restricts
to the fragment without division and square root, the overall computational power,
i.e. the sets decided, of computational trees and decision trees are the same. 
However, while testing wether a given polynomial is greater than $0$ need only 
one node in an algebraic decision tree, in general it requires more in algebraic 
computational trees since one needs to compute the polynomial explicitly from
basic algebraic operations.

\begin{figure}
  \begin{tikzpicture}
    \node (start) [shape=rounded rectangle,draw] {start};
    \node[below=0.5cm] at (start.south) (f1) [shape=rounded rectangle,draw]
    {\small $f_1 = x_1- x_2$};
    \draw (f1) to (start);
    \node[below=0.5cm] at (f1.south) (f2) [shape=rounded rectangle,draw] {\small
      $f_2 = x_1- x_3$};
    \draw (f2) to (f1);
    \node[below=0.5cm] at (f2.south) (f3) [shape=rounded rectangle,draw] {\small
      $f_3 = x_2- x_3$};
    \draw (f3) to (f2);
    \node[below=0.5cm] at (f3.south) (f4) [shape=rounded rectangle,draw] {\small
      $f_4 = f_1 \times f_2$};
    \draw (f4) to (f3);
    \node[below=0.5cm] at (f4.south) (f5) [shape=rounded rectangle,draw] {\small
      $f_5 = f_4 \times f_3$};
    \draw (f5) to (f4);
    \node[below=0.5cm] at (f5.south) (test) [shape=rounded rectangle,draw] {\small
      $f_5 = 0$};
    \draw (test) to (f5);
    \node[below=1cm,right=1cm] at (test.south) (if1) [shape=rounded
    rectangle,draw] {false};
    \node[below=1cm,left=1cm] at (test.south) (if2) [shape=rounded
    rectangle,draw] {true};
    \draw (if1) to (test);
    \draw (if2) to (test);
  \end{tikzpicture}
  \caption{An algebraic computation tree}
  \label{fig:act}
\end{figure}

Given an integer $k\in\omega$, we define the following subspaces of 
$\realN^{\omega}$:
\begin{itemize}
\item $\realN^{\omega}_{k\geqslant 0}=\{(x_{1},\dots,x_{k},\dots)\in
	\realN^{\omega}\mid x_{k}\geqslant 0\}$;
\item $\realN^{\omega}_{k\leqslant 0}=\{(x_{1},\dots,x_{k},\dots)\in
	\realN^{\omega}\mid x_{k}\leqslant 0\}$;
\item $\realN^{\omega}_{k> 0}=\{(x_{1},\dots,x_{k},\dots)\in
	\realN^{\omega}\mid x_{k}> 0\}$;
\item $\realN^{\omega}_{k< 0}=\{(x_{1},\dots,x_{k},\dots)\in
	\realN^{\omega}\mid x_{k}< 0\}$;
\item $\realN^{\omega}_{k=0}=\{(x_{1},\dots,x_{k},\dots)\in
	\realN^{\omega}\mid x_{k}= 0\}$;
\item $\realN^{\omega}_{k\neq 0}=\{(x_{1},\dots,x_{k},\dots)\in
	\realN^{\omega}\mid x_{k}\neq 0\}$.
\end{itemize}

      

\begin{definition}[treeings] 
A \emph{treeing} is an acyclic and finite graphing, i.e. a graphing $F$ for which 
there exists a finite graphing representative $T$ with set of control states 
$\Space{S^{T}}=\{0,\dots,s\}$ and such that every edge of $T$ is state-increasing, 
i.e. for each edge $e$ of source $S_{e}$, for all $x\in S_{e}$, 
\[ \pi_{\Space{S^{T}}}(\alpha(m_{e})(x)>\pi_{\Space{S^{T}}}(x),\] where 
$\pi_{\Space{S^{T}}}$ denotes the projection onto the control states space.

A \emph{computational graphing} is a graphing $T$  with distinguished states 
$\top$, $\bot$ which admits a finite representative such that each edge $e$ has 
its source equal to one among 
$\realN^{\omega}$, 
$\realN^{\omega}_{k\geqslant 0}$, 
$\realN^{\omega}_{k\leqslant 0}$, 
$\realN^{\omega}_{k> 0}$, 
$\realN^{\omega}_{k< 0}$, 
$\realN^{\omega}_{k=0}$, and 
$\realN^{\omega}_{k\neq 0}$.

A \emph{computational treeing} is a treeing $T$ which is a computational graphing
with the distinguished states $\top$, $\bot$ being incomparable maximal elements 
of the state space.
\end{definition}

% Je suis resté le plus proche possible de la définition de Ben-Or, même si je
% ne l'aime pas tant que ça
\begin{definition}[Algebraic computation trees, {\cite{Ben-Or83}}]
  An \emph{algebraic computation tree} on $\realN^n$ is a binary tree $T$ with a
  function that assigns:
  \begin{itemize}
  \item to any vertex $v$ with only one son (simple vertex) an operational
    instruction of the form
    \begin{align*}
      f_v &= f_{v_i} \circ f_{v_j}\\
      f_v &= c \circ f_{v_i}\\
      f_v &= \sqrt{f_{v_i}}
    \end{align*}
    where $\circ \in \{ +, -, \times, /\}$, ${v_i}, {v_j}$ are ancestors of $v$
    and $c\in \realN$ is a constant;
  \item to any vertex $v$ with two sons a test instruction of the form
    \begin{align*}
      f_{v_i} &> 0\\
      f_{v_i} &= 0\\
      f_{v_i} &\geqslant 0
    \end{align*}
    where $v_i$ is an ancestor of $v$ or $f_{v_i} \in \{x_1,\dots,x_n\}$;
  \item to any leaf an output $\texttt{YES}$ or $\texttt{NO}$.
  \end{itemize}
\end{definition}

An algebraic computational tree is represented in Figure \ref{fig:act}.

Let $W \subseteq \realN^n$ be any set and $T$ be an algebraic computation
tree. We say that $T$ computes the membership problem for $W$ if for all $x \in
\realN^n$, the traversal of $T$ following $x$ ends on a leaf labelled
\texttt{YES} if and only if $x\in W$.


%We can then define the \amc of algebraic computation trees. The underlying space
%is $\realN^{n+\ell}$ and the acting monoid is generated by $\boadd{i}{j}{k}$,
%$\bosubstract{i}{j}{k}$, $\bomultiply{i}{j}{k}$, $\bodivide{i}{j}{k}$,
%$\boadd{i}{c}{j}$, $\bosubstract{i}{c}{j}$, $\bomultiply{i}{c}{j}$,
%$\bodivide{i}{c}{j}$, $\bosquareroot{i}{j}$, for $n <i \leqslant n+\ell$,
%$0 <j,k < n+\ell$ and $c\in\realN$ acting on $\realN^{n+\ell}$ through
%\begin{itemize}
%\item $\alpha(\boadd{i}{j}{k})(x_1,\dots,x_{n+\ell}) = (x_1, \dots, x_{i-1}, x_j
%  + x_k, x_{i+1}, \dots, x_{n+\ell})$;
%\item $\alpha(\bosubstract{i}{j}{k})(x_1,\dots,x_{n+\ell}) = (x_1, \dots, x_{i-1}, x_j
%  - x_k, x_{i+1}, \dots, x_{n+\ell})$;
%\item $\alpha(\bomultiply{i}{j}{k})(x_1,\dots,x_{n+\ell}) = (x_1, \dots, x_{i-1}, x_j
%  \times x_k, x_{i+1}, \dots, x_{n+\ell})$;
%\item $\alpha(\bodivide{i}{j}{k})(x_1,\dots,x_{n+\ell}) = (x_1, \dots, x_{i-1}, x_j
%  / x_k, x_{i+1}, \dots, x_{n+\ell})$ if $x_k \neq 0$;
%\item $\alpha(\boadd{i}{c}{k})(x_1,\dots,x_{n+\ell}) = (x_1, \dots, x_{i-1}, c
%  + x_k, x_{i+1}, \dots, x_{n+\ell})$;
%\item $\alpha(\bosubstract{i}{c}{k})(x_1,\dots,x_{n+\ell}) = (x_1, \dots, x_{i-1}, c
%  - x_k, x_{i+1}, \dots, x_{n+\ell})$;
%\item $\alpha(\bomultiply{i}{c}{k})(x_1,\dots,x_{n+\ell}) = (x_1, \dots, x_{i-1}, c
%  \times x_k, x_{i+1}, \dots, x_{n+\ell})$;
%\item $\alpha(\bodivide{i}{c}{k})(x_1,\dots,x_{n+\ell}) = (x_1, \dots, x_{i-1}, c
%  / x_k, x_{i+1}, \dots, x_{n+\ell})$ if $x_k \neq 0$;
%\item
%  $\alpha(\bosquareroot{i}{k})(x_1,\dots,x_{n+\ell}) = (x_1, \dots, x_{i-1},
%  \sqrt{x_k}, x_{i+1}, \dots, x_{n+\ell})$ if $x_k \geqslant 0$.
%\end{itemize}

We can define the \amc of algebraic computation trees. The underlying space
is $\realN^{\omega}$ and the acting monoid is generated by $\boadd{i}{j}{k}$,
$\bosubstract{i}{j}{k}$, $\bomultiply{i}{j}{k}$, $\bodivide{i}{j}{k}$,
$\boadd{i}{c}{j}$, $\bosubstract{i}{c}{j}$, $\bomultiply{i}{c}{j}$,
$\bodivide{i}{c}{j}$, $\bosquareroot{i}{j}$, for $i,j,k\in\omega$ and $c\in\realN$
 acting on $\realN^{\omega}$ as follows:
\begin{itemize}
\item $\alpha(\boadd{i}{j}{k})(x_1,\dots,x_{i-1},x_{i},x_{i+1},\dots) = (x_1, \dots, 
x_{i-1}, x_j  + x_k, x_{i+1}, \dots)$;
\item $\alpha(\bosubstract{i}{j}{k})(x_1,\dots,x_{i-1},x_{i},x_{i+1},\dots) = (x_1, 
\dots, x_{i-1}, x_j  - x_k, x_{i+1}, \dots)$;
\item $\alpha(\bomultiply{i}{j}{k})(x_1,\dots,x_{i-1},x_{i},x_{i+1},\dots) = (x_1, 
\dots, x_{i-1}, x_j  \times x_k, x_{i+1}, \dots)$;
\item $\alpha(\bodivide{i}{j}{k})(x_1,\dots,x_{i-1},x_{i},x_{i+1},\dots) = (x_1, 
\dots, x_{i-1}, x_j  / x_k, x_{i+1}, \dots)$ if $x_k \neq 0$;
\item $\alpha(\boadd{i}{c}{k})(x_1,\dots,x_{i-1},x_{i},x_{i+1},\dots) = (x_1, 
\dots, x_{i-1}, c  + x_k, x_{i+1}, \dots)$;
\item $\alpha(\bosubstract{i}{c}{k})(x_1,\dots,x_{i-1},x_{i},x_{i+1},\dots) = (x_1, 
\dots, x_{i-1}, c  - x_k, x_{i+1}, \dots)$;
\item $\alpha(\bomultiply{i}{c}{k})(x_1,\dots,x_{i-1},x_{i},x_{i+1},\dots) = (x_1, 
\dots, x_{i-1}, c  \times x_k, x_{i+1}, \dots)$;
\item $\alpha(\bodivide{i}{c}{k})(x_1,\dots,x_{i-1},x_{i},x_{i+1},\dots) = (x_1, 
\dots, x_{i-1}, c  / x_k, x_{i+1}, \dots)$ if $x_k \neq 0$;
\item
  $\alpha(\bosquareroot{i}{k})(x_1,\dots,x_{i-1},x_{i},x_{i+1},\dots) = (x_1, 
  \dots, x_{i-1}, \sqrt{x_k}, x_{i+1}, \dots)$ if $x_k \geqslant 0$.
\end{itemize}

\begin{definition}
Let $T$ be a computational treeing on the \amc of algebraic computational 
trees. The set of inputs $\inputs{T}$ (resp. outputs $\outputs{T}$) is the set 
of integers $k$ (resp. $i$) such that there exists an edge $e$ in $T$:
\begin{itemize} 
\item either $e$ is realised by one of $\boadd{i}{j}{k}$, $\boadd{i}{k}{j}$,
$\bosubstract{i}{j}{k}$, $\bosubstract{i}{k}{j}$, $\bomultiply{i}{j}{k}$, 
$\bomultiply{i}{k}{j}$, $\bodivide{i}{j}{k}$, $\bodivide{i}{k}{j}$
$\boadd{i}{c}{k}$, $\bosubstract{i}{c}{k}$, $\bomultiply{i}{c}{k}$,
$\bodivide{i}{c}{k}$, $\bosquareroot{i}{k}$;
\item or the source of $e$ is one among 
$\realN^{\omega}_{k\geqslant 0}$, 
$\realN^{\omega}_{k\leqslant 0}$, 
$\realN^{\omega}_{k> 0}$, 
$\realN^{\omega}_{k< 0}$, 
$\realN^{\omega}_{k=0}$, and 
$\realN^{\omega}_{k\neq 0}$.
\end{itemize}

The \emph{input space} $\inputspace{T}$ of a treeing $T$ on the \amc of 
algebraic computational trees is defined as the set of indices $k\in\omega$ 
belonging to $\inputs{T}$ but not to $\outputs{T}$.
\end{definition}

\begin{definition}
Let $T$ be a treeing on the \amc of computational trees, and let $n$ be an
integer larger than the maximal element in $\inputspace{T}$. We say that 
$T$ computes the membership problem for $W\subseteq\realN^{n}$ if for 
all $(x_1,\dots, x_n) \in \realN^n$, the successful iterations of $T$ on the 
subspace $\{(y_1,\dots, y_n,\dots)\in\realN^{\omega}\mid\forall 1\geqslant i
\geqslant n, y_i=x_i\}\times\{0\}$ reach the state $\top$ if and only if 
$x\in W$.
\end{definition}

\begin{remark}
Consider two elements $a,b,$ in $\{(y_1,\dots, y_n,\dots)\in\realN^{\omega}
\mid\forall 1\geqslant i\geqslant n, y_i=x_i\}\times\{0\}$. One can easily check
that $\pi_{\Space{S}}(T^{n}(a))=\top$ if and only if $\pi_{\Space{S}}(T^{n}(b))
=\top$, where $\pi_{\Space{S}}$ is the projection onto the state space and 
$T^{n}(a)$ represents the $n$-th iteration of $T$ on $a$. It is therefore
possible to consider only a standard representative of $(x_1,\dots, x_n) \in 
\realN^n$, for instance $(x_1,\dots, x_n,0,0,\dots) \in \realN^\omega$, to
decide whether $(x_1,\dots, x_n) \in \realN^n$ is accepted by $T$.
\end{remark}

\begin{definition}
  Let $T$ be an algebraic computation tree on $\realN^{n}$, and $T^{\circ}$ 
  be the associated directed acyclic graph, built from $T$ by merging all the 
  leaves tagged $\texttt{YES}$ in one leaf $\top$ and all the leaves tagged 
  $\texttt{NO}$ in one leaf $\bot$. Suppose the internal vertices are numbered
  $\{n+1,\dots, n+\ell \}$; the numbers $1,\dots,n$ being reserved for the input.

  We define $[T]$ as the graphing with control states
  $\{n+1,\dots, n+\ell, \top, \bot \}$ and where each internal vertex $i$ of
  $T^{\circ}$ defines either:
  \begin{itemize}
  \item a single edge of source $\realN^{\omega}$ realized by:
    \begin{itemize}
    \item $(\boadd{i}{j}{k}, i \mapsto t)$ if $i$ is associated to $f_{v_i} =
      f_{v_j} + f_{v_k}$ and $t$ is the son of $i$;
    \item $(\bosubstract{i}{j}{k}, i \mapsto t)$ if $i$ is associated to $f_{v_i} =
      f_{v_j} - f_{v_k}$ and $t$ is the son of $i$;
    \item $(\bomultiply{i}{j}{k}, i \mapsto t)$ if $i$ is associated to $f_{v_i} =
      f_{v_j} \times f_{v_k}$ and $t$ is the son of $i$;
    \item $(\boadd{i}{c}{k}, i \mapsto t)$ if $i$ is associated to $f_{v_i} =
      c + f_{v_k}$ and $t$ is the son of $i$;
    \item $(\bosubstract{i}{c}{k}, i \mapsto t)$ if $i$ is associated to $f_{v_i} =
      c - f_{v_k}$ and $t$ is the son of $i$;
    \item $(\bomultiply{i}{c}{k}, i \mapsto t)$ if $i$ is associated to $f_{v_i} =
      c \times f_{v_k}$ and $t$ is the son of $i$;
    \end{itemize}
  \item a single edge of source $\{(x_1,\dots,x_{n+\ell},\dots) \in 
  \realN^{\omega} \mid x_k \neq 0 \}$ realized by:
    \begin{itemize}
    \item $(\bodivide{i}{j}{k}, i \mapsto t)$ if $i$ is associated to
      $f_{v_i} = f_{v_j} / f_{v_k}$ and $t$ is the son of $i$;
    \item $(\bodivide{i}{c}{k}, i \mapsto t)$ if $i$ is associated to
      $f_{v_i} = c / f_{v_k}$ and $t$ is the son of $i$;
    \end{itemize}
  \item a single edge of source $\realN^{\omega}_{k\geqslant 0}\times\{i\}$ 
  realized by $(\bosquareroot{i}{k}, i \mapsto t)$ if $i$ is associated to 
  $f_{v_i} = \sqrt{f_{v_k}}$ and $t$ is the son of $i$;
  \item a pair of edges:
    \begin{itemize}
    \item one of source
      $\realN^{\omega}_{k> 0}\times \{i\}$
      realized by $(\identity, i \mapsto j)$ and one of source
      $\realN^{\omega}_{k\leqslant 0}\}
      \times \{i\}$ realized by $(\identity, i \mapsto k)$ if $i$ is associated to 
      $f_{v_i} >0$ and its two sons are $j$ and $k$;
    \item one of source
      $\realN^{\omega}_{k\geqslant 0}\times \{i\}$ realized by $(\identity, 
      i \mapsto j)$ and one of source
      $\realN^{\omega}_{k< 0}\times 
      \{i\}$ realized by $(\identity, i \mapsto k)$ if $i$ is associated to
      $f_{v_i} \geqslant 0$ and its two sons are $j$ and $k$;
    \item one of source
      $\realN^{\omega}_{k= 0}\times 
      \{i\}$ realized by $(\identity, i \mapsto j)$ and one of source
      $\realN^{\omega}_{k\neq 0}\times
      \{i\}$ realized by $(\identity, i \mapsto k)$ if $i$ is associated to
      $f_{v_i} >0$ and its two sons are $j$ and $k$;
    \end{itemize}
  \end{itemize}
\end{definition}

\begin{proposition}
Let $\alpha$ be the \amc of algebraic computation trees. Then any algebraic 
computation tree $T$ is faithfully interpreted as an $\alpha$-graphing $[T]$.
I.e. $T$ computes the membership problem for $W\subseteq\realN^{n}$ if
and only if $[T]$ computes the membership problem for $W$.

Moreover, $[T]$ is a computational treeing, and for any computational treeing
$G$ computing the membership problem for $W\subseteq\realN^{n}$, 
there exists an algebraic computation tree $T_{W}$ computing the membership
problem for $W$.
\end{proposition}

\begin{proof}
%\textcolor{red}{I commented the previous (draft of) proof. TO DO.}
A computation tree defines a graphing $[T]$, and the
natural graphing representative obtained from the inductive definition of $[T]$
is clearly a treeing because $T$ is a tree. That this treeing represents faithfully
the computational tree $T$ raises no difficulty.

Let us now show that the membership problem of a subset $W\subseteq\realN^n$
that can be decided by a computational treeing is also decided by an algebraic
computational tree $T$. We prove the result by induction on the number of states of the
computational treeing. The initial case is when $T$ the set of states is exactly $\{1,\top,
\bot\}$ with the order defined by $1<\top$ and $1<\bot$ and no other relations. This 
computational treeing has at most 2 edges, since it is deterministic and the source 
of each edge is a subset among 
$\realN^{\omega}$, 
$\realN^{\omega}_{k\geqslant 0}$, 
$\realN^{\omega}_{k\leqslant 0}$, 
$\realN^{\omega}_{k> 0}$, 
$\realN^{\omega}_{k< 0}$, 
$\realN^{\omega}_{k=0}$, and 
$\realN^{\omega}_{k\neq 0}$. 

We first treat the case when there is only one edge of
source $\realN^n$. An element $(x_1,\dots,x_n)\in\realN^n$ is decided by $T$ if the 
main representative $((x_1,\dots,x_n,0,\dots),1)$ is mapped to $\top$. Since there is
only one edge of source the whole space, either this edge maps into the state $\top$ 
and the decided subset $W$ is equal to $\realN^n$, or it maps into $\bot$ and the 
subset $W$ is empty. In both cases, there exists an algebraic computational tree
deciding $W$. For the purpose of the proof, we will however construct a specific 
algebraic computation tree, namely the one that first computes the right expression
and then accepts or rejects. I.e. if the only edge is mapping into $\top$ (resp. $\bot$)
is realised by an element $m$ in the \amc of algebraic computation trees which can 
be written as a product of generators $g_1,\dots,g_k$, we construct the tree of height 
$k+1$ that performs (in that order) the operations corresponding to $g_1$, $g_2$, etc., 
and then answers "yes" (resp. "no").

Now, the case where there is one edge of source a strict subspace, e.g. 
$\realN^{\omega}_{k\geqslant 0}$ (all other cases are treated in a similar manner)
and mapping into $\top$ (the other case is treated by symmetry). First, let us remark 
that if there is no other edge, one could very well add an edge to $T$ mapping into 
$\bot$ and realised by the identity with source the complementary subspace 
$\realN^{\omega}_{k< 0}$. We build a tree as follows. First, we test whether the 
variable $x_k$ is greater or equal to zero; this node has two sons corresponding to
whether the answer to the test is "yes" or "no". We now construct the two subtrees
corresponding to these two sons. The branch corresponding to "yes" is described
by the edge of source $\realN^{\omega}_{k\geqslant 0}$: we construct the tree of 
height $k+1$ performing the operations corresponding to the generators $g_1$, 
$g_2$, etc. whose product defined the realiser $m$ of $e$, and then answers "yes"
(resp. "no") if the edge $e$ maps into the state $\top$ (resp. $\bot$). Similarly, the 
other subtree is described by the realiser of the edge of source 
$\realN^{\omega}_{k< 0}$.

The result then follows by induction, plugging small subtrees as described above 
in place of the leaves of smaller subtrees.
\end{proof}

\subsection{Random Access Machines (\srams)}
In this paper, we will consider algebraic parallel random access machines, that
act not on strings of bits, but on integers. In order to define those properly,
we first define the notion of (sequential) random access machine (\sram) before
considering their parallelisation.

A \sram \emph{command} is a pair $(\ell, I)$ of a \emph{label} (or \emph{line})
$\ell \in \naturalN^{\star}$ and a \emph{command} $\command{I}$ among the
following:
\[
\begin{array}{rclll}
  \textrm{Commands} & := & \Skip; & \command{X_{i} \coloneqq c};
  & \command{X_{i} \coloneqq X_{j} \circ X_{k}};\\
                    && \command{X_{i} \coloneqq X_{j}};
                         &\command{X_{i} \coloneqq \sharp{}X_{j}};
                                  &\command{\sharp{X_{i}}\coloneqq X_{j}};\\
                    &&\multicolumn{3}{l}{\conditional{X_i = 0}{\ell}{\ell'};}
\end{array}
\]
where $i, j \in \naturalN$, $\circ \in \{+, -, \times, / \}$, $c\in \integerN$
is a constant and $\ell, \ell' \in \naturalN^{\star}$ are labels.

A \sram \emph{machine} $M$ is then a finite set of commands such that the set of
labels is $\{1,2,\dots,\length{M}\}$, with $\length{M}$ the \emph{length} of
$M$. We will denote the commands in $M$ by $(i,\instr{i})$, i.e. $\instr{i}$
denotes the $i$-labelled command.

The semantics of \sram machines is quite straightforward: a configuration is
represented as a pair $(i,\sigma)$ where $i$ is the current label and
$\sigma: \naturalN\rightarrow\integerN$ -- an eventually null function --
represent the state of the registers. Then the commands above are easily
interpreted as a transition to the label $i+1$ (except in case of the
conditional) and an updated function $\sigma$. E.g. a
$\command{\sharp X_{i}\coloneqq X_{j}}$ command induces the following
transition: $(i,\sigma) \rightarrow (i+1,\sigma[\sigma(j)/\sigma(i)])$, while a
$\command{X_{i}\coloneqq \sharp X_{j}}$ command induces the transition
$(i,\sigma) \rightarrow (i+1,\sigma[\sigma(\sigma(j))/i])$.

We now define the \sram action. As we intend to consider \prams, we consider
from the begining the memory of a \sram to be separated in two infinite blocks
$\integerN^{\omega}$, intended to represent both \emph{shared} and a
\emph{private} memory cells. The underlying space is % the space of functions
$\Space{X}= % \integerN^{d}\rightarrow
\integerN^{\omega}\times\integerN^{\omega}$.
% it is thought of as the result of applying a sequence of instructions to an
% initial configuration defined from $\integerN^{d}$. 
The set of generators is defined following the possible actions of an \sram on
the memory: $\boconst{i}{c}$, $\boadd{i}{j}{k}$, $\bosubstract{i}{j}{k}$,
$\bomultiply{i}{j}{k}$, $\boeuclidivide{i}{j}{k}$, $\copyy{i}{j}$,
$\refcopy{i}{j}$, $\copyref{i}{j}$.
%
Each of the generator acts as follows (we do not distinguish the two kinds of
memory and suppose the indices unique here):
\begin{itemize}[nolistsep,noitemsep]
\item
  $\alpha(\boconst{i}{c})(x_1,\dots,x_{i-1},x_{i},x_{i+1},\dots) =
  (x_{1},\dots,x_{i-1},c,x_{i+1},\dots)$;
\item
  $\alpha(\boadd{i}{j}{k})(x_1,\dots,x_{i-1},x_{i},x_{i+1},\dots) =
  (x_{1},\dots,x_{i-1},x_{j}+x_k,x_{i+1},\dots)$;
\item $\alpha(\bosubstract{i}{j}{k})(x_1,\dots,x_{i-1},x_{i},x_{i+1},\dots) =
  (x_{1},\dots,x_{i-1},x_{j}-x_k,x_{i+1},\dots)$;
\item $\alpha(\bomultiply{i}{j}{k})(x_1,\dots,x_{i-1},x_{i},x_{i+1},\dots) =
  (x_1, \dots, x_{i-1}, x_j \times x_k, x_{i+1}, \dots)$
\item for $\alpha(\boeuclidivide{i}{j}{k})$,
  \[(x_1,\dots,x_{i-1},x_{i},x_{i+1},\dots) \mapsto
    \left\{
      \begin{array}{ll}
        (x_1, \dots, x_{i-1}, b, x_{i+1}, \dots)& \text{such that }x_j = b
                                                  x_k +r \\
                                                &\text{and }
                                                  0\leqslant r < x_k\\
                                                &\text{if }
                                                  x_k \neq 0\\
        (x_1, \dots, x_{i-1}, 0, x_{i+1}, \dots)& \text{else}
      \end{array}
    \right.
  \]
\item
  $\alpha(\copyy{i}{j})(x_1,\dots,x_{i-1},x_{i},x_{i+1},\dots) =
  (x_{1},\dots,x_{i-1},x_{j},x_{i+1},\dots)$;
\item $\alpha(\refcopy{i}{j})(x_1,\dots,x_{i-1},x_{i},x_{i+1},\dots) =
  (x_{1},\dots,x_{i-1},x_{x_{j}},x_{i+1},\dots)$;
\item
  $\alpha(\copyref{i}{j})(x_1,\dots,x_{i-1},x_{i},x_{i+1},\dots) =
  (x_{1},\dots,x_{x_{i}-1},x_{j},x_{x_{i}+1},\dots)$.
\end{itemize}

\sram machines can be represented as graphings w.r.t. this action; intuitively
the encoding works as follows. The notion of \emph{control state} allows to
represent the notion of \emph{line} in the program. Then, the action just
defined allows for the representation of all commands but the conditionals. The
conditionals are represented as follows: depending on the value of $X_{i}$ one
wants to jumps either to the line $\ell$ or to the line $\ell'$; this is easily
modelled by two different edges of respective sources
$\hyperplan{i}=\{\vec{x}~|~ x_{i}=0\}$ and
$\complementset{\hyperplan{i}}=\{\vec{x}~|~ x_{i}\neq0\}$.

\begin{definition}
  Let $M$ be a \sram machine. We define $[M]$ as the graphing with set of
  control states $\{0,1,\dots,L,L+1\}$ where each line $\ell$ defines:
  \begin{itemize}[nolistsep,noitemsep]
  \item either a single edge $e$ of source $\Space{X}\times\{\ell\}$ and realised
    by:
    \begin{itemize}[nolistsep,noitemsep]
    \item $(\identity,\ell\mapsto \ell+1)$ if $\instr{\ell}$ is \Skip;
    \item $(\boconst{i}{c},\ell\mapsto \ell+1)$ if $\instr{\ell}$ is
      $\command{X_i \coloneqq c}$;
    \item $(\boadd{i}{j}{k},\ell\mapsto \ell+1)$ if $\instr{\ell}$ is
      $\command{X_i \coloneqq X_j + X_k}$;
    \item $(\bosubstract{i}{j}{k},\ell\mapsto \ell+1)$ if $\instr{\ell}$ is
      $\command{X_i \coloneqq X_j - X_k}$;
    \item $(\bomultiply{i}{j}{k},\ell\mapsto \ell+1)$ if $\instr{\ell}$ is
      $\command{X_i \coloneqq X_j \times X_k}$;
    \item $(\copyy{i}{j},\ell\mapsto \ell+1)$ if $\instr{\ell}$ is
      $\command{X_{i} \coloneqq X_{j}}$;
    \item $(\copyref{i}{j},\ell\mapsto \ell+1)$ if $\instr{\ell}$ is
      $\command{X_{i}\coloneqq \sharp X_{j}}$;
    \item $(\refcopy{i}{j},\ell\mapsto \ell+1)$ if $\instr{\ell}$ is
      $\command{\sharp{}X_{i} \coloneqq X_{j}}$;
    \end{itemize}
  \item a single edge $e$ of source $\hyperplan{k}\times\{\ell\}$ and realised
    by $(\boeuclidivide{i}{j}{k},\ell\mapsto \ell+1)$ if $\instr{\ell}$ is
    $\command{X_i \coloneqq X_j/X_k}$;
  \item or, if the line is a conditional
    $\command{if~X_{i}=0~goto~\ell^{0}~else~\ell^{1}}$, a pair
    $e,\complementset{e}$ of edges of respective sources
    $\hyperplan{i}\times\{\ell\}$ and $\complementset{\hyperplan{i}}\times\{\ell\}$
    and realised by respectively $(\identity,\ell\mapsto \ell^{0})$ and
    $(\identity,\ell\mapsto \ell^{1})$.
  \end{itemize}
\end{definition}

If a graphing $T$ in the \amc of \srams has a distinguished control state
$\top$, we say that $T$ \emph{accepts} $x\in \integerN^d$ if $T$ accepts
$((d,x_1, \dots, x_d, 0, \dots), (0,\dots) , (0, \dots), \dots)$.

One can now easily check that the representation of the machine $M$ as a
graphing is sound. % A map
% $\theta: \integerN^{d}\rightarrow\integerN^{\omega}\times\integerN^{\omega}$ is
% a \emph{parametrisation of the input}: for each element
% $\vec{a}\in\integerN^{d}$, $\theta(\vec{a})$ represents a configuration of the
% memory blocks.
% Starting from any such configuration seen as the \emph{initial
%   configuration}, the iteration $[M]_{L}^{k}(\theta)$ yields a new configuration
% $\theta_{k}$ which is such that $\theta_{k}(\vec{a})$ coincides with the
% configuration $M^{k}(\theta(\vec{a}))$.


\begin{theorem}\label{thm:soundsram}
  The representation of \srams as graphings is sound.
\end{theorem}

\begin{proof}
  The proof is an easy verification that the interpretation of commands in the
  graphing do coincide with the semantics of these commands.
\end{proof}

\subsection{The Crew}

\paragraph{Parallel Random Access Machines (\prams).} Based on the notion of
\sram, we are now able to consider their parallelisation, namely \prams. A \pram
machine $M$ is simply given as a finite sequence of \sram machines
$M_{1},\dots,M_{p}$, where $p$ is the number of \emph{processors} of $M$. Each
processor $M_{i}$ has access to its own, private, set of registers
$(\command{X}_{k}^{i})_{k\geqslant 0}$ and a \emph{shared memory} represented as
a set of registers $(\command{X}_{k}^{0})_{k\geqslant 0}$.

As usual, one has to deal with conflicts when several processors try to access
the shared memory simultaneously. We here chose to work with the \crew
discipline, i.e. \emph{Concurrent Read, Exclusive Write}, implemented as
follows: at a given step at which several processors try to write in the shared
memory, only the processor with the smallest index will be allowed to do so. In
order to model such parallel computations, we abstract the \crew at the level of monoids

, by performing
an operation reminiscent (in that it also generalizes the free product) of the
amalgamated sum \cite[A, I, \S 7, 3]{Bourbaki:AlgI-III}, but chosen relatively
to monoid actions. For this, we suppose that we have two monoid actions
$\MonGaR{G}{R}\acton \Space{X}\times\Space{Y}$ and
$\MonGaR{H}{Q}\acton \Space{X}\times\Space{Z}$, where $\Space{X}$ represents the
shared memory. Among the generators of each monoid, we will separate those that
potentially conflict with the generator of the other monoid (typically a write)
from the other and perform a sum over those generators.

\begin{definition}[Conflicted sum]
  Let $\MonGaR{G}{R}$, $\MonGaR{G'}{R'}$ be two monoids and
  $\# \subseteq G \times G'$ a relation between the generators of $G$ and $G'$,
  called the \emph{conflict} relation, we define the \emph{conflicted sum of
    $\MonGaR{G}{R}$ and $\MonGaR{G'}{R'}$ over $\#$}, noted
  $\MonGaR{G}{R} \ast_{\#} \MonGaR{G'}{R'}$,as the monoid
  $\MonGaR{(\{1\} \times G) \cup (\{2\} \times G')}{Q}$ where $Q$ is defined as:
  \[ Q=(\{1\} \times G) \cup (\{2\} \times G') \cup \{ \big((1,g)(2,g'),
    (2,g')(1,g) \big), (g,g') \notin \# \} \cup \{ (\mathbf{1}, e)\} \cup \{
    (\mathbf{1}, e')\} \]
  where $\mathbf{1}$, $e$ and $e'$ are the neutral elements of
  $\MonGaR{G}{R} \ast_{\#} \MonGaR{G'}{R'}$ and its two components.

  In the particular case where $\# = (G \times H') \cup (H \times G')$, with
  $H, H'$ respectively subsets of $G$ and $G'$, we will write the sum
  $\MonGaR{G}{R}\ncproduct{H}{H'}\MonGaR{G'}{R'}$.
\end{definition}

\begin{remark}
  When the conflic relation $\#$ is empty, this defines the usual direct product
  of monoids. This was to be expected. Indeed, one should think of this relation as
  representing the elements that do not commute because they interact with the
  shared memory. As a consequence, when it is empty no conflicts can arise
  w.r.t. the shared memory. In other words, the direct product of monoids
  corresponds to the parallelisation of processes \emph{without shared memory}.

  Dually, when the relation full ($\# = G \times G'$), it defines the free
  product of the monoids, so the free product corresponds to the parallelisation
  of processes where all instructions interact with the shared memory.
\end{remark}

% We abstract the \crew mode of interaction at the level of monoid, by performing
% a particular amalgamated sum\footnote{The terminology is not unified here:
%   indeed, the amalgamated sum of groups is the generalization of the free
%   products, hence the name \emph{free product with amalgamation} is also
%   used. We prefer this name, as it is a sum in the category-theoretic sense.}
% \cite[A, I, \S 7, 3]{Bourbaki:AlgI-III} relative to monoid actions. We define it
% for two \amc, the general case being obtained by induction. For this, we suppose
% that we have two monoid actions $\MonGaR{G}{R}\acton \Space{X}\times\Space{Y}$
% and $\MonGaR{H}{Q}\acton \Space{X}\times\Space{Z}$, where $\Space{X}$ represents
% the shared memory. Among the generators of each monoid, we will separate those
% that potentially conflict with the generator of the other monoid (typically a
% write) from the other and perform the amalgamated sum over those generators.

% \begin{definition}[amalgamated sum]
%   Let $\MonGaR{G}{R}$, $\MonGaR{G'}{R'}$ be two monoids and
%   \[ h : A \to \MonGaR{G}{R} \qquad h' : A \to \MonGaR{G'}{R'} \] be two monoid
%   morphisms. The \emph{sum of $\MonGaR{G}{R}$ and $\MonGaR{G'}{R'}$ amalgamated
%     by $A$}, noted $\MonGaR{G}{R} \ast_A \MonGaR{G'}{R'}$, is defined as the
%   monoid
%   $\MonGaR{(\{1\} \times G) \cup (\{2\} \times G')}{Q}$ where $Q$ is defined as:
%   \[ Q=(\{1\} \times G) \cup (\{2\} \times G') \cup \{
%     \left((1,h(a)),(2,h'(a))\right), a \in A \} \cup \{ (\mathbf{1}, e)\} \cup
%     \{ (\mathbf{1}, e')\} . \]
%   where $\mathbf{1}$, $e$ and $e'$ are the neutral
%   elements of $\MonGaR{G}{R} \ast_A \MonGaR{G'}{R'}$ and its two components.  
% \end{definition}





\begin{definition}
  Let $\alpha: M\acton\Space{X}\times \Space{Y}$ be a monoid action. We say that
  an element $m\in M$ is \emph{central relatively to $\alpha$} (or just
  \emph{central}) if the action of $m$ commutes with the first projection
  $\pi_{X}:\Space{X}\times \Space{Y}\rightarrow\Space{X}$,
  i.e. $\alpha(m);\pi_{X}=\alpha(m)$; in other words $m$ acts as the identity on
  $\Space{X}$.
%  \begin{commutativediagram}{1}{5}{1}
%    {
%      X \times Y \& \& X \times Y\\
%      \& X\\
%    };
%    \path[-stealth]
%    (m-1-1) edge [auto] node {$m$} (m-1-3)
%    (m-1-1) edge [auto] node [below] {$\pi_1$} (m-2-2)
%    (m-1-3) edge [auto] node {$\pi_1$} (m-2-2);
%  \end{commutativediagram}
%
%  The set of central elements of $M$ is the \emph{centre} $Z(M)$ of $M$.
\end{definition}

Intuitively, central elements are those that will not affect the shared memory. As such, they do not raise any issues when the processes are put in parallel. On the other hand, \emph{non-central elements} need to be dealt with care. 

\begin{definition}
Let $\MonGaR{G}{R}\acton \Space{X}\times\Space{Y}$ be an \amc. We note $Z_{\alpha}$ the set of central elements and $\bar{Z}_{\alpha}(G)$ the set $\{m\in G~|~ n\not\in Z_{\alpha}\}$.
\end{definition}

% We will now define the \crew operation on \amc. We first define an operation on monoids that will allow for the definition of the \crew action later on.

% \begin{definition}[Noncommutative Product]\label{def:noncommprod}
% Let $\MonGaR{G}{R}$ and $\MonGaR{G'}{R'}$ be representations of monoids, and let $H\subseteq G$ and $H'\subseteq G'$ be subsets of generators. We define the noncommutative product of $\MonGaR{G}{R}$ and $\MonGaR{G'}{R'}$ above $H,H'$ as the monoid $\MonGaR{G\times G'}{R\times \Id\cup \Id\times R'\cup Q}$ where $Q$ is defined as:
% \[ Q=\{(a,a')(b,b')=(aa',bb')~|~ a,a'\not\in H\text{ or }b,b'\not\in H'\}. \]
% The resulting monoid is denoted $\MonGaR{G}{R}\ncproduct{H}{H'}\MonGaR{G'}{R'}$.
% \end{definition}

% \begin{remark}
% When both $H,H'$ are empty, this defines the usual product of monoids. This was to be expected. Indeed, one should think of $H,H'$ as representing the set of elements that are not central, i.e. that write on the shared memory. As a consequence, when $H,H'$ are empty no conflicts can arise w.r.t. the shared memory. In other words, the product of monoids corresponds to the parallelisation of processes \emph{without shared memory}.
% \end{remark}

\begin{definition}[The \crew operation]
Let $\alpha: \MonGaR{G}{R}\acton \Space{X}\times\Space{Y}$ and $\beta: \MonGaR{H}{Q}\acton \Space{X}\times\Space{Z}$ be \amcs. We define the \amc 
\[\crew(\alpha,\beta): \MonGaR{G}{R}\ncproduct{\bar{Z}_{\alpha}(G)}{\bar{Z}_{\beta}(G')}\MonGaR{G'}{R'}\acton \Space{X}\times\Space{Y}\times\Space{Z}\] 
by letting $\crew(\alpha,\beta)(m,m')=\alpha(m)\ast\beta(m')$ on elements of $G\times G'$, where $\alpha(m)\ast\beta(m')$ is defined as:
\begin{eqnarray*}
\lefteqn{\alpha(m)\ast\beta(m'): \Space{X}\times\Space{Y}\times\Space{Z}\rightarrow\Space{X}\times\Space{Y}\times\Space{Z}} \\
&=\left\{
\begin{array}{ll}
\Delta;[\alpha(m);\pi_{Y},\beta(m')]  & \text{ if $m\not\in\bar{Z}_{\alpha}(G), m'\in\bar{Z}_{\beta}(G')$;}\\
\Delta;[\alpha(m),\beta(m');\pi_{Z}] & \text{ otherwise }
\end{array}
\right.
\end{eqnarray*}
with $\Delta: (x,y,z)\mapsto(x,y,x,z): \Space{X}\times\Space{Y}\times\Space{Z}\rightarrow\Space{X}\times\Space{Y}\times\Space{X}\times\Space{Z}$.
\end{definition}

We now need to check that we defined the operation on monoids and the action coherently. In other words, that the previous operation is compatible with the quotient by the adequate relations, i.e. it does define a monoid action.

\begin{lemma}
The \crew operation on \amcs is well-defined.
\end{lemma}
% \begin{proof}
% We check that the definition above extends to a monoid action, i.e. the mapping just defined is coherent with the relations introduced in Definition \ref{def:noncommprod}. To see this, it is sufficient to notice that only the relations in the set $Q$ may lead to incoherences. But those are exactly the relations of the type $(m,m')(n,n')=(mm,nn')$ for which $(\alpha(m)\ast\beta(m'));(\alpha(n)\ast\beta(n'))=(\alpha(mn)\ast\beta(m'n'))$. For instance, one can easily check that if $m',n'\not\in\bar{Z}_{\beta}(G')$ the maps $\Delta;[\alpha(m),\beta(m');\pi_{Z}];\Delta;[\alpha(n),\beta(n');\pi_{Z}]$ and $\Delta;[\alpha(mn),\beta(m'n');\pi_{Z}]$ are equal.
% \end{proof}


% The crew operation is actually an elaboration of the two fundamental
% observations: parallelism creates non-commutativity and ``a non-commutative
% space engenders its own time'' \cite{Connes}.

\subsection{The crew of the \sram action: \prams}

We can now define \amc of \prams and thus the interpretations of \prams as
abstract programs. For each integer $p$, we define the \amc $\crew^{k}(\alpha)$
for $\alpha$ is the \amc for \srams defined in the previous section. This allows
the consideration of up to $p$ parallel \srams. The interpretation of such a
\sram with $p$ processors is then defined by considering a set of states equal
to $L_{1}\times L_{2}\times \dots \times L{p}$ where for all $i$ the set $L_{i}$
is the set of labels of the $i$-th processor.

Now, to deal with arbitrary large \prams, i.e. with arbitrarily large number of
processors, one considers the following \amc defined as a \emph{direct limit}.

\begin{definition}[The \amc of  \prams]
  Let $\alpha: M\acton\Space{X\times X}$ be the \sram{}
  \amc. % \footnote{Note that to use the crew operation, we need to split the
  % space between public and private registers; we do not provide the full
  % definition of this \amc since it is not necessary for this definition
  % and the full definition is provided in the previous section.}
  The \amc of \prams is defined as $\varinjlim\crew^{k}(\alpha)$, where
  $\crew^{k-1}(\alpha)$ is identified with a restriction of $\crew^{k}(\alpha)$
  through
  $\crew^{k-1}(\alpha)(m_{1},\dots,m_{k-1})\mapsto
  \crew^{k}(\alpha)(m_{1},\dots,m_{k-1},1)$.
\end{definition}

Remark that the underlying space of the \pram{} \amc is defined as the union
\( \cup_{n\in \omega} \integerN^{\omega} \times (\integerN^{\omega})^n\) which
we will write \( \integerN^{\omega} \times (\integerN^{\omega})^{(\omega)}\).

The fact that the \crew operation on actions does define the semantics of the
\crew discipline for concurrent read/write should be clear from the
definitions. As a consequence, Theorem \ref{thm:soundsram} the interpretation of
\prams as graphings is sound.

\begin{theorem}
  The representation of \prams as graphings is sound.
\end{theorem}

% \textcolor{red}{This should be quick. Maybe we can delete this subsection and
% simply explain how \prams are represented, and state a soundness result here.}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> IGprograms.tex <==
\section{Abstract Models of Computation, Abstract Progams}

The basic intuitions here can be summarised by the following slogan: "Computation, as a dynamical process, can be modelled as a dynamical system". Of course, the above affirmation cannot be true of all computational processes; for instance the traditional notion of dynamical system is deterministic. In practice, one works with a generalisation of dynamical systems named \emph{graphings}; introduced as part of a family of models of linear logic, graphings have been shown to model non-deterministic and probabilistic computation.



Given a set $G$, we denote by $\FreeMon{G}$ the free monoid on $G$, i.e. the set of finite sequences of elements of $G$.

\begin{definition}
We recall that a \emph{presentation} $\GaR{G}{R}$ of a monoid $M$ is given by a set $G$ of \emph{generators} and a set $\relations{R}$ of \emph{relations} such that $M$ is isomorphic to $\FreeMon{G}/\relations{R}$.
\end{definition}

\begin{definition}
  Let $M$ be a monoid and $\Space{X}$ be a space. An action of $M$ on $\Space{X}$
  is a monoid morphism $\alpha$ from $M$ to the set of endomorphisms on $\Space{X}$.
  We denote actions by $\alpha: M \acton \Space{X}$, sometimes omitting the morphism $\alpha$.
\end{definition}
In this definition, we purposely chose to not specify the kind of space considered. As a consequence, if one considers a discrete space $\Space{X}$ (i.e. sets), the set of endomorphisms will simply be the set of functions $\Space{X}\rightarrow\Space{X}$. Similarly, if $\Space{X}$ is a topological space, the set of endormorphisms will be continuous maps (hence $\alpha$ will be a \emph{continuous action}). Etc.


\begin{definition}
An \emph{abstract model of computation} (\amc) is defined as a triple $(G,\relations{R},\alpha)$, where $\GaR{G}{R}$ is a presentation of a monoid $\MonGaR{G}{R}$ and $\alpha$ is a monoid action $\MonGaR{G}{R}\acton \Space{X}$.
We denote an \amc as $\AMC[X]{G}{R}{\alpha}$.
\end{definition}

\begin{remark}
Although it might seem enough to define an abstract model of computation solely as a monoid action, the choice of a presentation of the monoid by generators and relations is important. First, when considering several models of computation, one wants to consider a notion of \emph{compilation}: an element $f\in \EndSp{Y}$ is compilable in the action $M\acton \Space{X}$ when there is an automorphism $\Psi:\Space{X}\rightarrow\Space{Y}$ such that one can write $X=\disjun_{i=1,\dots, n} X_{i}$ and the restriction of $\Psi^{-1}\circ f\circ \Psi$ to $X_{i}$ is the restriction of an element $g_{i}$ of $M$ to $X_{i}$. To use this notion of compilation in a meaningful way, one would want to quantify the \emph{complexity} of compilation. This can be done only by considering a definition of the monoid $M$ as generators and relations $\GaR{G}{R}$, allowing one to consider the \emph{degree}\footnote{Let us notice that this notion has already been considered in relation to dynamical systems, used to define what is called the \emph{algebraic entropy} and the \emph{fundamental group entropy} \cite[Section 3.1]{KatokHasselblatt}} of $g_{i}$ -- the length of the smallest word in $G^{\ast}$ representing $g_{i}$ -- and therefore the degree of the compilation of $f$ into $\AMC{G}{R}{\alpha}$.

Although we will not consider the notion of compilation in this work, it is remarkable that the representation of the monoid as generators and relations is needed in the definition of the \emph{parallelisation of actions} -- defined as the \crew operation.
\end{remark}

\begin{definition}
A graphing representative $G$ w.r.t. a monoid action $M\acton\Space{X}$ is defined as a set of \emph{edges} $E^{G}$ and for each element $e\in E^{G}$ a pair $(S^{G}_{e},m^{G}_{e})$ of a subspace $S^{G}_{e}$ of $\Space{X}$ -- the \emph{source} of $e$ -- and an element $m^{G}_{e}\in M$ -- the \emph{realiser} of $e$.
\end{definition}

Graphings come in different flavours (discrete, topological, measurable), depending on the type of space $\Space{X}$ one wishes to consider. If $\Space{X}$ is a topological space, the action will be \emph{continuous}, if $\Space{X}$ is a measure space, the action will be \emph{measurable}. While the notion of graphing representative does not depend on this choice, the notion of \emph{graphing} is defined as a quotient of the space of graphing representative w.r.t. an adequate notion of equivalence. We will here consider the notion of \emph{topological graphing} \cite{seiller-igg}, which we will simply call \emph{graphings}. In this case, the notion of equivalence is easier to define than in the case of \emph{measurable graphings} as the latter requires one to consider almost-everywhere equality.

% \Luc{Je ne comprends plus la définition de raffinement : la bijection $\theta$
%   est de quoi dans quoi ? $E^F \to E^G$, plutôt ? Mais dans ce cas, j'ai du mal
%   à voir en quoi les partitions pourraient avoir plus d'un élément ?
% %
%   Je rate un truc ?}
%   \Thomas{Non, tu as raison. La definition telle qu'elle apparait ci-dessous n'a pas trop de sens. La bijection $\theta$ n'a pas lieu d'être. Ce que tu veux, c'est une partition de $E^{G}$ qui soit $E^{F}$-indexée. Avec l'idée que les sources des elements de $E^G$ correspondant à un $f\in E^F$ soient disjointes (up to ensemble de mesure nulle) et que leur union soit la source de $f$, que les fonctions réalisant toutes ces arêtes et leurs poids coincident avec la fonction réalisant $f$ et avec le poids de $f$ respectivement.\newline
%   En regardant le papier sur les graphages, il y a effectivement une fonction $\theta$, mais elle n'est pas demandée biejctive. Est-ce que tu as pris la definition depuis deux sources différentes? (Ou bien est-ce que c'est moi qui ai mis cette definition dans un moment de fatigue?) Je pense que la definition dans le récent papier TOCL (non-deterministic automata) est la plus propre et la plus simple; je la colle juste après celle qui ne va pas. (Comme ça tu vois les deux, et on peut chercher si cela pose des problèmes de notations plus loin,)}

% \begin{definition}[Refinement]
% Let $F,G$ be graphing representatives. Then $F$ is a refinement of $G$, noted $F\leqslant G$, when there exists a bijection $\theta: S^{F}\rightarrow S^{G}$ and an $E^{G}$-indexed partition $(E^{F}_{g})_{g\in E^{G}}$ of $E^{F}$ such that for all $g\in E^{G}$, the family $(S^{F}_{f})_{f\in E^{F}_{g}}$ is a partition of $S^{G}_{g}$ and for all $f\in E^{F}_{g}$ we have $m^{G}_{g}=m^{F}_{f}$.

% This notion defines an equivalence relation defined by $F\sim G$ if and only if there exists $H$ with $H\leqslant F$ and $H\leqslant G$.
% \end{definition}

\begin{definition}[Refinement]
A graphing representative $F$ is a refinement of a graphing representative $G$,
noted $F\leqslant G$, if there exists a partition\footnote{We allow the sets
  $E^{F}_{e}$ to be empty.} $(E^{F}_{e})_{e\in E^{G}}$ of $E^{F}$ such that
$\forall e\in E^{G}$:
$$
\left(\cup_{f\in E^{F}_{e}} S^{F}_{f} \right) \mathbin{\triangle}
S^{G}_{e} = \emptyset;
\hspace{1cm} 
\forall f\neq f'\in E^{F}_{e},\quad S^{F}_{f} \mathbin{\triangle}
S^{F}_{f'} = \emptyset;
$$
$$
\forall f\in E^{F}_{e},\quad m^{F}_{f}=m_{e}^{G}
$$
This notion defines an equivalence relation defined by $F\sim G$ if and only if
there exists $H$ with $H\leqslant F$ and $H\leqslant G$.
\end{definition}

\begin{definition}
A \emph{graphing} is an equivalence class of graphing representatives w.r.t. the
equivalence relation generated by refinements.

A graphing is \emph{deterministic} if its representatives are deterministic, i.e. if any representative $G$ is such that for all $x\in\Space{X}$ there is at most one $e\in\ E^{G}$ such that $x\in S^{G}_{e}$.
\end{definition}

\begin{definition}
An \emph{abstract program} $A$ within an \amc $\AMC{G}{R}{\alpha}$ is defined as a finite set $\Space{S^{A}}$ of \emph{control states} and a graphing $G^{A}$ w.r.t. the monoid action $\MonGaR{G}{R}\times\mathfrak{S}_{k}\acton \Space{X}\times\Space{S^{A}}$.

An abstract program is \emph{deterministic} if its underlying graphing is deterministic.
\end{definition}


==> context.tex <==


\noindent\textbf{Lower Bounds and Barriers in Computational Complexity.}
%
%\noindent\textbf{Computational Complexity.}
%The field of computational complexity was initiated soon after the conception of the first computers. 
%While theoretical results had already established a definition of the notion of "computable function" 
%on the set of natural numbers, it became quickly apparent that computable did not mean practical, 
%as many functions considered computable could not be computed within a reasonable time. (Example?)
%
%The first complexity class defined was that of \emph{feasible functions} 
%\cite{hartmanisstearns,cobham,edmonds65}, which is now known as  $\Ptime$: the set of polynomial 
%time computable functions, i.e. functions $f$ for which there exists a polynomial $p$ and a machine $M$ 
%computing $f$ whose running time on an input $n$ is bounded by $p(n)$. This class, apart from being 
%the first ever complexity class to appear in the literature, is arguably the most important one in computer 
%science. Many fundamental problems concern its relation to other classes, such as $\NPtime$ which is 
%the extension of $\Ptime$ if one allows for non-deterministic machines in the above definition. These 
%problems, however, are still open.
%(lower bounds, barriers)
%
%Beyond the relationship between \Ptime and other classes, the general question of \emph{classifying} 
%the complexity classes became one of the main objectives of the field, and a number of important results 
%were obtained within the first years. \newline
%%However, as researchers continued working on separation, the question continuously more and more complex.
%
%
%\noindent\textbf{Separation, Lower bounds and Barriers}
As part of the classification problem, complexity theory has traditionally been
concerned with proving \emph{separation results}. Among the numerous open
separation problems lies the much advertised \Ptime vs. \NPtime problem of
showing that some problems considered hard to solve but efficient to verify do
not have a polynomial time algorithm solving them.

Proving that two classes $B\subset A$ are not equal can be reduced to 
finding lower bounds for problems in $A$: by proving that certain problems cannot be solved with less than certain
resources on a specific model of computation, one can show that two classes are not equal.
Conversely, proving a separation result $B\subsetneq A$ provides a lower bound for the 
problems that are $A$\emph{-complete} \cite{cooknpcomplete} -- i.e. problems that are in some way \emph{universal} for 
the class $A$.

%The central and most well-known


%The proven lower bound results are however very few, and most separation problems
%remain as generally accepted conjectures. For instance, a proof that the class
%of non-deterministic exponential problems is not included in what is thought of
%as a very small class of circuits was not achieved until very recently
%\cite{Williams}.
%
% [Barriers, GCT and the Mulmuley paper]

The failure of most techniques of proof has been studied in itself, which lead
to the proof of the existence of negative results that are commonly called
\emph{barriers}. Altogether, these results show that all proof methods we know
are ineffective with respect to proving interesting lower bounds. Indeed, there
are three barriers: relativisation \cite{relativization}, natural proofs
\cite{naturality} and algebrization \cite{algebraization}, and every known proof
method hits at least one of them. This shows the need for new 
methods\footnote{In the words of S. Aaronson and A. Wigderson 
\cite{algebraization}, \enquote{We speculate that going beyond this limit 
[algebrization] will require fundamentally new methods.}}. However, to this day, 
only one research program aimed at proving new separation results is commonly 
believed to have the ability to bypass all barriers: Mulmuley and
Sohoni's Geometric Complexity Theory (\gct) program
\cite{GCTsurvey2}.\newline



\noindent\textbf{Algebraic models and Geometric Complexity Theory.}
%(TODO: A paragraph on how things are different in algebraic models.)
Geometric Complexity Theory (\gct) is widely considered to be a promising 
research program that might lead to separation results based on algebraic 
geometry. 
It is also widely believed to necessitate
new and extremely sophisticated pieces of mathematics in order to achieve its goal. 
The research program aims to
prove the \Ptime $\neq$ \NPtime lower bound by showing that certain algebraic
surfaces (representing the permanent and the discriminant, which are believed
\cite{Valiant} to have different complexity if \Ptime $\neq$ \NPtime) cannot be
embedded one into the other. Although this program has lead to interesting
developments as far as pure mathematics is concerned, it has not enhanced
our understanding of complexity lower bounds for the time being and, even
according to Mulmuley himself, such understanding may not be obtained in the 
near future \cite{100years}. Moreover, recent negative results \cite{Ikenmeyer} have 
closed the easiest path towards it promised by \gct.

The \gct program was inspired, according to its creators, by a lower bound
result obtained by Mulmuley \cite{Mulmuley99}. Specifically, it was proved that
the \maxflow problem (deciding whether a certain quantity can flow from a source
to a target in a weighted graph) is not solvable efficiently in a specific
parallel model ("\pram without bit operations"). The \maxflow problem is quite
interesting as it is known to be in \Ptime (by reduction to linear programming,
or the Ford-Fulkerson algorithm \cite{FordFulkerson}), and even \Ptime-complete
for logspace Turing reductions \cite{MaxflowComplete}. This lower bound proof, 
despite being the main inspiration of the well-known \gct research program, remains
seldom cited and has not led to variations applied to other problems. At first
sight it relies a lot on algebraic geometric techniques and results, such as the
Milnor-Thom theorem\footnote{We note here that, even though this is not
  mentionned by Mulmuley, the Milnor-Thom theorem was previously used in
  lower bounds proofs by, e.g. Dobkin and Lipton \cite{DobkinLipton76}, Steele
  and Yao \cite{SteeleYao82}, Ben-Or \cite{Ben-Or83}, Cucker \cite{Cucker92}.}.
 

\noindent\textbf{Parallel computation and Mulmuley's result}

(A paragraph on parallel computation)

(A paragraph on NC vs Ptime)

(A paragraph on Mulmuley's model of computation with a formal definition)

(A paragraph on mulmuley's theorem (statement) and proof)\newline

\noindent\textbf{Our main results}

(A paragraph on our method)

(A paragraph on how it abstracts Steele and Yao, Cucker and Mulmuley)

(A paragraph on Steele and Yao vs Ben-Or)

(A paragraph on our model of computation with a formal definition)

(A paragraph on our theorem (statement) and proof)

% \subsection{Plan of the paper}

% (SUGGESTION)
% \begin{itemize}
% \item Section 1/2. Introductions courtes et longues (Thomas/écrire; deadline 6 septembre; Luc/relire deadline 20 septembre) 
% \item Section 3. Programs as dynamical systems (Luc/exemples à ajouter; deadline 6 septembre; Thomas/relire deadline 13 septembre)
% \item Section 4. Entropy and cell decompositions (--)
% \item Section 5. Steele and Yao (--)
% \item Section 6. Cucker (Luc/écrire deadline 6 septembre; Thomas/relire deadline 13 septembre)
% \item Section 7. Mulmuley (Thomas/relire;Luc/relire)
% \item Section 8. Ben Or and entropic co-trees (--)
% \item Section 9. Main result (Thomas/Luc deadline 20 septembre)
% \item Section 10. Conclusion (deadline 20 septembre)
% \end{itemize}



==> mulmuley.tex <==
\section{\srams and \prams}

% In this section, we will define a specific monoid action \sram and show that
% \sram machines correspond to (deterministic) \emph{graphings} w.r.t. this monoid
% action. We first recall what graphings are and how they are used here as
% mathematical models of computation. We then introduce the \sram action and show
% how machines are represented as graphings.


\subsection{The entropic co-trees of a \pram}

A \pram defines a family of entropic co-trees by using Def.
\ref{def:co-tree}. These co-trees are in the \amc of \prams, which we designed
to be similar to the \amc of algebraic computation trees. The three main
differences are:
\begin{itemize}
\item the \amc of \prams acts on $\integerN^{\omega} \times
  (\integerN^{\omega})^{(\omega)}$, while that algebraic computational trees
  acts on $\realN^d$;
\item an action of the \amc of \prams with $p$ processors is a tuple of $p$
  actions in the \amc of \srams;
\item the euclidian division in the \amc of \prams can not be translated
  straightforwardly.
\end{itemize}

We will handle this difficulties separately, by introducing an \amc of \prams
over $\realN$ and translating a treeing in the \amc of \prams into a treeing in
the \amc of \prams over $\realN$, and then by adapting the proofs of Section
above to this \amc.

\paragraph{\prams over $\realN$}

The \amc of \srams over $\realN$ is defined as the \amc of \srams, but the
underlying space is
$\realN^{\omega} \times \realN^{\omega} \times \realN^{\omega}$, where we
interpret the first two copies as public and the third as private, and the
generator corresponding to euclidian division is replaced by the real
division. we introduce the second public copy so as to be able to have fresh
variables: indeed, we cannot define the set of memory cells that a program can
use, due to the indirect addressing $\command{\sharp{X_{i}}\coloneqq X_{j}}$.

Explicitly the set of generators is given by: $\boconst{i}{c}$,
$\boadd{i}{i}{j}$, $\bosubstract{i}{i}{j}$, $\bomultiply{i}{i}{j}$,
$\bodivide{i}{i}{j}$, $\copyy{i}{j}$, $\refcopy{i}{j}$, $\copyref{i}{j}$ that
act by:
\begin{itemize}[nolistsep,noitemsep]
\item
  $\alpha(\boconst{i}{c})(x_1,\dots,x_{i-1},x_{i},x_{i+1},\dots) =
  (x_{1},\dots,x_{i-1},c,x_{i+1},\dots)$;
\item
  $\alpha(\boadd{i}{i}{j})(x_1,\dots,x_{i-1},x_{i},x_{i+1},\dots) =
  (x_{1},\dots,x_{i-1},x_{i}+x_j,x_{i+1},\dots)$;
\item $\alpha(\bosubstract{i}{i}{j})(x_1,\dots,x_{i-1},x_{i},x_{i+1},\dots) =
  (x_{1},\dots,x_{i-1},x_{i}-x_j,x_{i+1},\dots)$;
\item $\alpha(\bomultiply{i}{i}{j})(x_1,\dots,x_{i-1},x_{i},x_{i+1},\dots) =
  (x_1, \dots, x_{i-1}, x_i \times x_j, x_{i+1}, \dots)$
\item
  $\alpha(\bodivide{i}{i}{j})= (x_1,\dots,x_{i-1},x_{i},x_{i+1},\dots) =
  (x_1, \dots, x_{i-1}, x_i/x_j, x_{i+1}, \dots)$ if $x_j \neq 0$;
\item
  $\alpha(\copyy{i}{j})(x_1,\dots,x_{i-1},x_{i},x_{i+1},\dots) =
  (x_{1},\dots,x_{i-1},x_{j},x_{i+1},\dots)$;
\item $\alpha(\refcopy{i}{j})(x_1,\dots,x_{i-1},x_{i},x_{i+1},\dots) =
  (x_{1},\dots,x_{i-1},x_{x_{j}},x_{i+1},\dots)$ if $x_j \in \omega$;
\item
  $\alpha(\copyref{i}{j})(x_1,\dots,x_{i-1},x_{i},x_{i+1},\dots) =
  (x_{1},\dots,x_{x_{i}-1},x_{j},x_{x_{i}+1},\dots)$ if $x_i \in \omega$.
\end{itemize}
The \amc of \pram over $\realN$ is then defined as the limit of the crew of this
\amc, just as in the $\integerN$ case, and so acts on
$\realN^{\omega} \times \realN^{\omega} \times (\realN^{\omega})^{(\omega)}$.


We do not define the \prams in this \amc, as we are just interested in it to
translate treeings. If a graphing $T$ in the \amc of \prams over $\realN$ has a
distinguished control state $\top$, we say that $T$ \emph{accepts}
$x\in \realN^d$ if $T$ accepts
$((d,x_1, \dots, x_d, 0, \dots), (0,\dots) , (0, \dots), \dots)$.

\paragraph{From a treeing of \pram to a treeing of \pram over $\realN$}

We can associate to every treeing in the \amc of \prams a treeing in the \amc of
\prams over $\realN$, that, limited to the integers, decide the same set.

In what follow, we will distinguish the copies on which a \pram acts by writing
$\vec{x} = ((x_1,\dots),(y_1,\dots),(z_1^i)_{0\leq i}) \in \realN^{\omega}
\times \realN^{\omega} \times (\realN^{\omega})^{(\omega)}$ the different
elements.

\begin{definition}
  Let $T$ be a treeing in the \amc of \prams with control states $S$, and
  suppose that its edges labelled with $\boeuclidivide{i}{j}{k}$ are numbered
  $1, \dots, t$.
  
  We define the \emph{real mate} $\realN(T)$ as the treeing with control states
  $S \times \{1,2,3\}$ where the $n$-th vertex labelled
  $\boeuclidivide{i}{j}{k}: a \to b$ is replaced by the vertices:
  \begin{itemize}
  \item one of source $a \cap \{\vec{x} \mid y_{2n} \geq 0\}$ and labelled by
    identity;
  \item one of source $a \cap \{\vec{x} \mid y_{2n} < x_k\}$ and labelled by the
    identity;
  \item one of source $a$ labelled by $\bosubstract{y_{2n+1}}{j}{y_{2n}}$
  \item one of source $a$ labelled by $\bodivide{i}{y_{2n+1}}{k}$
  \end{itemize}
  where the state moves in all these operations in its new component.
\end{definition}

The real mate allows to compute the euclidian division when restricted to
integers, by adding new variables and relations between them.

\begin{theorem}
  \label{thm:mulmuley-co-tree}
  Let $T$ be a \pram with $p$ processors, that ends in $k$ steps.

  The real mate of its $k$-th entropic co-tree is a treeing $Q$ in the \amc of
  \prams over $\realN$ such that:
  \begin{itemize}
  \item $Q$ is of height at most $4k$;
  \item $\forall x \in \integerN^d$, $Q$ accepts $x$ if and only if $T$ accepts
    $x$;
  \item the subspace accepted by this treeing can be defined by a set of
    $(2p)^{4k}$ polynomial equations of degree at most $2^{4k}$.
  \end{itemize}
\end{theorem}
\begin{proof}
  The only point that needs to be developed is the last one: we traverse the
  tree and add equations as for the algebraic computation trees.
\end{proof}

We remark here that we could add a square root instruction to our \prams, just
as in the algebraic computation trees. (TODO: A faire dans la version longue.)

==> surfaces.tex <==
\section{Separation of fans}
\subsection{Algebraic Surfaces}
\label{sec:alg-surfaces}

An algebraic surface in $\realN^3$ is a surface defined by an equation of the
form $p(x,y,z)=0$ where $p$ is a polynomial. If $S$ is a set of surfaces, each
defined by a polynomial, the \emph{total degree} of $S$ is defined as the sum of
the degrees of polynomials defining the surfaces in $S$.

Let $K$ be a compact of $\realN^3$ delimited by algebraic surfaces and $S$ be a
finite set of algebraic surfaces, of total degree $\delta$. We can assume that
$K$ is actually delimited by two affine planes of equation $z=\mu$ and
$z=2\mu_z$ and the cone of a rectangle
$\{ (x,y,1) \mid |x|, |y| \leqslant \mu_{x,y}\}$, by taking any such compact
containing $K$ and adding the surfaces bounding $K$ to $S$. $S$ defines a
partition of $K$ by considering maximal compact subspaces of $K$ whose
boundaries are included in surfaces of $S$. Such elements are called the
\emph{cells} of the decomposition associated to $S$.

The cell of this partition can have complicated shapes: in particular, a cell
can have a arbitrarily high number of surfaces of $S$ as boundaries. We are
going to refine this partition into a partition $\Collins{S}$ whose cells are
all bounded by cones of curves and at most two surfaces in $S$.

\subsection{Collins' decomposition}

We define the \emph{silhouette} of a surface defined by the equation
$p(x,y,z) = 0$ by:
\begin{align*}
  \left\{
  \begin{array}{l}
    p(x,y,z) = 0 \\
    x\frac{\partial p}{\partial x} + y \frac{\partial
    p}{\partial y} + z \frac{\partial p}{\partial z} = 0.
  \end{array}
  \right.
\end{align*}
The silhouette of a surface is the curve on the surface such that all points
$(x,y,z)$ of the silhouette are such that the ray $[(x,y,z)]$ is orthogonal to
the tangent plane of the surface on $(x,y,z)$.

Up to infinitesimal perturbation of the coefficients of the polynomials, we can
assume that the surfaces of $S$ have no integer points in $K$.

$\projectionAz{K} = \{ \projectionAz{x} \mid x \in K\}$ is a compact of the affine plane
$\AffinePlane$. Let us consider the set $\projectionAz{S}$ of curves in
$\projectionAz{K}$ containing:
\begin{itemize}[nolistsep,noitemsep]
\item the projection of the silhouettes of surfaces in $S$;
\item the projection of the intersections of surfaces in $S$ and of the
  intersection of surfaces in $S$ with the planes $z=\mu(1+\frac{n}{6\delta})$,
  $n \in \{1,\ldots,6\delta-1\}$, where $\delta$ is the total degree of $S$;
\item \emph{vertical lines} of the form $\{(x,a,1) \mid |x| \leq 2^{\beta+1} \}$
  for $a$ a constant such that such lines pass through:
  \begin{itemize}[nolistsep,noitemsep]
  \item all intersections among the curves;
  \item all singular points of the curves;
  \item all critical points of the curves with a tangent supported by
    $\vec{e}_y$.
  \end{itemize}
\end{itemize}
$\projectionAz{S}$ defines a Collins decomposition \cite{Collins:1975} of
$\projectionAz{K}$. The intersection of any affine line supported by $\vec{e}_y$ of
the plane with a region of this decomposition is connected if nonempty.

Let $c$ be a cell in $\projectionAz{S}$. It is enclosed by two curves in
$\projectionAz{K}$ and at most two vertical lines. The curves can be parametrized by
$c_{\max} : x \mapsto \max \{y \in \realN \mid (x,y,1) \in c \}$ and
$c_{\min} : x \mapsto \min \{y \in \realN \mid (x,y,1) \in c \}$, which are both
smooth functions. The \emph{volatility} of $c$ is defined as the number of
extrema of the second derivatives $c_{\min}''$ and $c_{\max}''$ on their domains
of definition.

\begin{figure}[t]
  \centering
  % \begin{asy}
  %   settings.outformat = "pdf";
  %   settings.render=16;
  %   size(200.0pt,0);
  %   import graph3;
  %   currentprojection = perspective(30*dir(75,0));
real r1=3, r0=2/3;
  %   int nu = 36, nv = 36;
  %   real theta = asin((2/3)/(18^(1/2)));
  %   real phi = pi/4;
  %   real rho = pi/2-(theta+phi);
  %   real r2= sin(phi-theta)/cos(phi-theta);
  %   real r3 = sin(phi+theta)/cos(phi+theta);
  %   path3 crossSection = Circle(r=r0, c=(r1,0,3), normal=Y, n= nu);
  %   pen colorFunction(int u, real theta) {
  %     real z = sin(u/nu * 2pi);
  %     real t = (z + 1) / 2;
return t*heavygray + (1-t)*lightgray;
  %   }
  %   pen colorFunction2(int u, real theta) {
  %     real z = sin(u/nu * 2pi);
  %     real t = (z + 1) / 2;
return (t*heavygray + (1-t)*lightgray)+opacity(0.4);
  %   }
  %   surface torus = surface(crossSection, c=(0,0,0), axis=Z, n=nv,
  %   angle1=90, angle2=390, color=colorFunction);
  %   surface torus2 = surface(crossSection, c=(0,0,0), axis=Z, n=nv,
  %   angle1=390, angle2=450, color=colorFunction2);
  %   draw(torus);
  %   draw(torus2);
  %   draw(-Z -- 5Z, gray, arrow=Arrow3(TeXHead2), L=Label("$z$",
  %   position=EndPoint));
  %   draw((0,(-1)*cos(phi-theta),(-1)*sin(phi-theta)) -- (0,(5.5)*cos(phi-theta),(5.5)*sin(phi-theta)), darkgray, arrow=Arrow3(TeXHead2), L=Label("$r_{1}$",
  %   position=EndPoint));
  %   draw((0,(-1)*cos(phi+theta),(-1)*sin(phi+theta)) -- (0,(5.5)*cos(phi+theta),(5.5)*sin(phi+theta)), darkgray, arrow=Arrow3(TeXHead2), L=Label("$r_{2}$",
  %   position=EndPoint));
  %   draw(Circle(r=r2, c=(0,0,1), normal=Z, n= nu));
  %   draw(Circle(r=r3, c=(0,0,1), normal=Z, n= nu));
  %   draw(Circle(r=2/3, c=(0,3,3), normal=X, n= nu));
  %   draw(scale3(6) * shift(-1/2,-1/2,1/6) * unitplane, surfacepen=lightgray+opacity(0.9));
  % \end{asy}
  \caption{A torus and the projection of its silhouette}
  \label{fig:torus-silhouette}
\end{figure}

This set of curves $\projectionAz{S}$ can be lifted to a set of surfaces
$\Collins{S}(K)$ of $K$ that contains:
\begin{itemize}[nolistsep,noitemsep]
\item the surfaces of $S$;
\item the cones $[s]$ of every curve $s$ in $\projectionAz{S}$;
\item the planes bounding $K$;
\item $6\delta-2$ \emph{dividing planes} of equation
  $z=\mu(1+\frac{n}{6\delta})$, $n \in \{1,\ldots,6\delta-1\}$.
\end{itemize}
The projection of a cell of $\Collins{S}$ is a cell of $\projectionAz{S}$. We
say that a cell of $\Collins{S}(K)$ is \emph{flat} if none of its boundaries are
included in surfaces of $S$.

Let us call $\Deg$ the number of cells in $\Collins{S}(K)$.

Let $c$ be a cell in $\Collins{S}(K)$. Its \emph{volatility} is defined as the
volatility of its projection in $\projectionAz{S}$.

\subsection{Volatility and Separation}
\label{subsec:volatility-separation}

\begin{definition}
  Let $K$ be a compact of $\realN^3$.
  
  A finite set of surfaces $S$ on $K$ \emph{separates} a $\rho$-fan $\Fan$ on
  $K$ if the partition on $\integerN^3 \cap K$ induced by $S$ is finer than the
  one induced by $\Fan$.
\end{definition}

\begin{theorem}
  \label{thm:mulmuley}
  Let $S$ be a finite set of algebraic surfaces of total degree $\delta$, and
  $\Fan$ a $\rho$-fan of bitsize $\beta$.

  If $S$ separates $\Fan$, there exists a compact $K$ and a cell of
  $\Collins{S}(K)$ with volatility greater than $\rho/\Deg$.
\end{theorem}

In order to prove this theorem, we will build explicitely the compact $K$ and
this cell by considering sample points on $\Fan$ and show in Lemma
\ref{lem:volatility} a bound on the volatility of this cell.

Let $K$ be a compact delimited by the cone of a rectangle
$\{ (x,y,1) \mid |x|, |y| \leqslant 2^{\beta+1}\}$ and two planes of equation
$z=\mu$ and $z=2\mu$, with $\mu>(6\delta+1)2^{\beta}$. We first remark that all
affine segments of $\Fan$ are in the rectangle base of $K$.

For each affine segment of $\Fan$ with endpoints $(x_i, y_1, 1)$ and
$(x_{i+1}, y_{i+1},1)$ let, for $0 < k < 10 \Deg$, $y_i^k$ be such that
$(x_i^k, y_i^k,1)$ is in the affine segment, where
$x_i^k = \frac{(10 \Deg-k)x_i + kx_{i+1}}{10 \Deg}$. We remark that, as
$|x_i-{x_{i+1}}| > 2^{-\beta}$, we have, for $k,k'$,
$|x_i^k - x_i^{k'}| > 2^{-\beta}/10\Deg$.

\begin{lemma}
  For all sample points $(x_i^k,y_i^k,1)$, there exists a flat cell in
  $\Collins{S}$ that contains an integer point of $[(x_i^k,y_i^k,1)]$.
\end{lemma}
\begin{proof}
  Let $(x_i^k,y_i^k,1)$ be a sample point. $[(x_i^k,y_i^k,1)]$ is divided in
  $N+1$ intervals by the dividing planes. On the other hand, $[(x_i^k,y_i^k,1)]$
  intersects surfaces of $S$ in at most $\delta$ points, by Bézout theorem. So,
  there exists an interval $e$ of $[(x_i^k,y_i^k,1)]$ that is bounded by the
  dividing planes and that do not intersect any surface in $S$. By construction,
  $e$ is included in a flat cell, and its projection on the $z$-axis has length
  $\mu/(6\delta+1)$, so, as $(x_i^k,y_i^k,1)$ is of bitsize $\beta$,
  $(n2^{\beta}x_i^k,n2^{\beta}y_i^k,n2^{\beta})$ is, for all $n\in \naturalN$ an
  integer point of the ray, so, as $\mu > (6\delta+1) 2^{\beta}$, $e$ contains
  an integer point.
\end{proof}

So, for each affine segment of $\Fan$, there exists a flat cell in
$\Collins{S}$ that contains integer points in the ray of at least $10$ sample
points of the affine segment. Going further, there exists a cell $c$ of
$\Collins{S}$ that contains integer points in the ray of at least 10 sample
points of $\rho/\Deg$ affine segments of $\Fan$.

% Let $c$ be such a cell and consider $\projectionAz{c}$, the projection of $c$ in the
% affine plane.
\begin{lemma}
  \label{lem:volatility}
  The volatility of $c$ is at least $\rho/\Deg$.
\end{lemma}

This is achieved by applying the mean value theorem on the function
$\projectionAz{c}_{\max}'$ on pairs of sample points. In particular, this proof
uses no algebraic geometry. % The details are in Appendix \ref{app:volatility}.

\begin{proof}
  Let $e$ be a segment of $\Fan$ such that the ray of 10 of its sample points
  contain an integer point in $c$. Let $p = (x,y,z)$ be one of its integer point
  and $\projectionAz{p}=(x_p,y_p,1)$ its projection, which is a sample point in
  $\projectionAz{c}$. Let $q=(x,y+1,z)$. As $\projectionAz{p}$ is in $\Fan$, and $S$
  separates $\Fan$, $q$ is not in $c$, and $\projectionAz{q} = (x_q,y_q,1)$ is not
  in $\projectionAz{c}$. By Thalès theorem, $0< y_q-y_p < \frac{1}{\mu}$. So, as
  $y_q > \projectionAz{c}_{\max}(x_p) > y_p$, we have in particular that
  $0< \projectionAz{c}_{\max}(x_p) - y_p < \frac{1}{\mu}$.

  So, the 10 sample points have coordinates that approximate the graph of
  $\projectionAz{c}_{\max}$ with an error bounded by $\frac{1}{\mu}$.  Consider two
  of them $p_1=(x_1,y_1,1)$ and $p_2=(x_2,y_2,1)$, such that $x_1<x_2$. Let $a$
  be the slope of $e$ (in particular $a=(y_2-y_1)/(x_2-x_1)$. By the mean value
  theorem, there exists $\alpha \in [x_1, x_2]$ such that
  $\projectionAz{c}_{\max}'(\alpha)=\frac{ \projectionAz{c}_{\max}(x_2) -
    \projectionAz{c}_{\max}(x_1) }{x_2-x_1}$. But
  $|\projectionAz{c}_{\max}(x_2) - \projectionAz{c}_{\max}(x_1)| \leq |y_2-y_1| +
  \frac{2}{\mu}$ and $|x_2-x_1| > \frac{1}{10\Deg 2^{\beta}}$. So,
  $|\projectionAz{c}_{\max}'(\alpha) - a| \leq 2 \frac{10\Deg 2^{\beta}}{\mu}$.

  So, the function $\projectionAz{c}_{\max}'$ is close to the value $a$, with error
  bounded, between all the sample points. By applying the mean value theorem
  again, we get that there exists a point in the interval such that
  $\projectionAz{c}_{\max}''$ is close to 0, with an error bounded by $2
  \frac{10\Deg 2^{\beta}}{\mu}$.

  In the same way, let $e'$ be another segment of $\Fan$ such that the ray of 10
  of its sample points contain an integer point in $c$, of slope $a'$. Let two
  of them be $p_1' = (x_1',y_1',1)$ and $p_2' = (x_2',y_2',1)$, and suppose
  $x_2'>x_1'>x_2$. By the same reasoning as above, there exists
  $\alpha' \in [x_1',x_2']$ such that
  $|\projectionAz{c}_{\max}'(\alpha') - a'| \leq 2 \frac{10\Deg 2^{\beta}}{\mu}$. By
  the mean value theorem, there exists $\beta \in [\alpha,\alpha']$ such that
  $\projectionAz{c}_{\max}''(\beta)=\frac{ \projectionAz{c}_{\max}'(\alpha') -
    \projectionAz{c}_{\max}'(\alpha) }{\alpha'-\alpha}>\frac{1}{\mu}(|a-a'|-2
  \frac{10\Deg 2^{\beta}}{\mu})$.

  So, for each of the $\rho/\Deg$ segments of $\Fan$, we can exhibit a point
  such that $\projectionAz{c}_{\max}''$ is close to zero, and for each successive
  segment, a point such that it is far. So $\projectionAz{c}_{\max}''$ has at least
  $\rho/\Deg$ extrema.
\end{proof}

\subsection{Volatility and Degree}
\label{subsec:volatility-degree}
Mulmuley's result follows from Thm. \ref{thm:mulmuley} and the two lemmas:
\begin{lemma}
  Let $S$ be a finite set of curves of total degree $\delta$, and $K$ be a
  compact. The cells of the decomposition $\Collins{S}$ of $K$ have a volatility
  bounded by a polynomial in $\delta$.
\end{lemma}
\begin{proof}
  Let $c$ be a cell in $\Collins{S}$ and $g(x,y)=0$ be the equation of one of
  the boundaries of $\projectionAz{c}$ in the affine plane. The degree of $g$ is
  bounded by the degree of the intersection of surfaces in $S$. Any extrema $x$
  of $f''$, where $f$ is a parametrization $y=f(x)$ of this boundary, can be
  represented as a point $(x,y,y^{(1)},y^{(2)},y^{(3)})$ in the 5-dimensional
  phase space that satisfy polynomial equations of the form:
  \begin{align*}
    g(x,y)=0,\qquad
    &g_1(x,y,y^{(1)})=0, \qquad
    g_2(x,y,y^{(1)},y^{(2)})=0\\
    &g_3(x,y,y^{(1)},y^{(2)},y^{(3)})=0, \qquad
    y^{(3)}=0,
  \end{align*}
  where all the polynomials' degrees are all bounded by the degree of the
  intersection of surfaces in $S$ (as they are the derivatives of $g$). So, by
  the Milnor--Thom theorem, such points are in number polynomial in the total
  degree of the surfaces of $S$.
\end{proof}

\begin{lemma}
  The number of cells $\Deg$ of the Collins decomposition of $S$ is polynomial
  in $\delta$.
\end{lemma}
\begin{proof}
  The intersection of the surfaces in $S$ are algebraic varieties of number
  bounded by $\delta$, by the Milnor--Thom theorem. Moreover, so are the
  silhouettes of the surfaces, as they are the intersection of two algebraic
  varieties of total degree smaller than $\delta$. So, the number of cells in
  $\Collins{S}$ is bounded by the number of cells of $S$ times the number of
  dividing planes times the number of intersections, silhouettes and vertical
  lines they engender.
\end{proof}

\begin{theorem}[Mulmuley]
  Let $S$ be a finite set of algebraic surfaces of total degree $\delta$.

  There exists a polynomial $P$ such that, for all $\rho > P(\delta)$, $S$ does
  not separate $\rho$-fans.
\end{theorem}

